RollingCache: Using Runtime Behavior to Defend Against Cache Side Channel Attacks

Shared caches are vulnerable to side channel attacks through contention in cache sets. Besides being a simple source of information leak, these side channels form useful gadgets for more sophisticated attacks that compromise the security of shared systems. The fundamental design aspect that contention attacks exploit is the deterministic nature of the set of addresses contending for a cache set. In this paper, we present RollingCache, a cache design that defends against contention attacks by dynamically changing the set of addresses contending for cache sets. Unlike prior defenses, RollingCache does not rely on address encryption/decryption, data relocation, or cache partitioning. We use one level of indirection to implement dynamic mapping controlled by the whole-cache runtime behavior. Our solution does not depend on having defined security domains, and can defend against an attacker running on the same or another core. We evaluate RollingCache on ChampSim using the SPEC-2017 benchmark suite. Our security evaluation shows that our dynamic mapping removes the deterministic ability to identify the source of contention. The performance evaluation shows an impact of 1.67\% over a mix of workloads, with a corresponding

==> security.tex <==
\section{Security Analysis}
\label{sec:security}
%\textcolor{blue}{The security of RollingCache built at two levels, the prime sequence is made more complex, and the probe is rendered non-indicative of the address set that was accessed.}
Launching contention-based attacks requires identifying the \emph{AddrSets} of interest and creating eviction sets for those \emph{AddrSets}~\cite{llcpractical}. 
%The state of the cache with mapping from \emph{AddrSets} to \emph{CacheSets} and number of misses prior to rollover for different \emph{AddrSets}, also referred to as the metadata, is unknown to the attacker. 
There are several properties of RollingCache that make it robust against these attacks at both the prime and probe stages. 
\begin{enumerate}
    \item The attacker does not know the number of accesses to an \emph{AddrSet} remaining before a pointer update/rollover to a new \emph{CacheSet}. 
    \item The eviction sets do not remain constant: they change as a function of cache replacement as multiple \emph{AddrSet}s point to the same \emph{CacheSet}.
    \item Random replacement can result in self-evictions. 
\end{enumerate}
%might not end up occupying the entirety of each \emph{CacheSet} associated with an \emph{AddrSet}, as a result of which the victim may go undetected. 
% so that a probe resulting in a miss may or may not be due to the victim. 
%, and so cannot be reused for an attack.  
At the prime stage, an attacker attempting to prime the cache will face the possibility of a rollover due to which its primed accesses can be lost even without victim accesses, and the victim may go undetected because of available space (property 1). At the same time, there is the possibility of self-eviction (property 3). 
At the probe stage, an attacker may incur additional misses due to self- and non-self-associative address accesses from the victim (property 2). Given the range of possible reasons for a miss, a miss at the probe stage does not indicate the victim's access to a self-associative address. 
We analyze each of these design aspects in detail in the following subsections, and show how learning an eviction set using known methods is both difficult and not useful for the attack. 

\subsection{Property I: Priming may not fill up CacheSets}
\label{security1}
Unlike a conventional cache, where the eviction set size is W (where W is the number of ways), the number of unique cache line accesses that form an eviction set in RollingCache is not known. The attacker does not know how many accesses from an \emph{AddrSet} remain before a pointer update, and therefore does not have the knowledge of how many accesses fill up the assigned \emph{CacheSets}. Consider the following scenarios, with W and 2W accesses. Let the number of ways in the cache be 4 (W = 4), and the \emph{AddrSet} under consideration be `X'. 

\begin{enumerate}
    \item Accessing W elements: It is possible that \emph{AddrSet} `X' has been accessed 2 times before the attacker attempts to prime values from an \emph{AddrSet}. The attacker's third access  will result in a pointer update. The attacker's previous cache fills will be reachable via \emph{PsPtr[X]}, and the attacker incurs no misses. The victim is able to bring data into the cache without detection. For instance, after 4 accesses from the attacker,  as shown in Figure~\ref{w2wnew}, the victim's access as 5 can go undetected, since all of the attacker's data is still accessible during probe.
    \item Accessing 2W elements: If there are no invalid cache blocks in \emph{PrPtr[X]}, the attacker may evict its own cache lines at random, as shown by 6 replacing 4 in Figure~\ref{w2wnew}. This is referred to as \emph{self eviction} during the prime stage. Secondly, a pointer update can occur midway, and result in a miss in an attacker's accesses even without the victim accessing \emph{AddrSet} `X', shown as 1 and 2 not being accessible after PtrUpdate 2 in Figure~\ref{w2wnew}. Thus, the attacker does not know which entries can be expected to incur a hit during probe.
\end{enumerate}


When the attacker probes the primed values, the misses from \emph{self eviction}, from having lost access to data due to 2 pointer updates, and from  fills by another \emph{AddrSet},  interfere with identifying the \emph{AddrSet} accessed by the victim. Further, the misses due to the attacker's probe are likely to trigger another pointer update, losing the work done toward priming.

\begin{figure}[tb]
\caption{Prime sequence for a 4 way set associative cache, using W or 2W accesses. White blocks represent invalid, grey represent valid cachelines from other \emph{AddrSets}, and red blocks represent attacker's accesses.}
\label{w2wnew}
\centering
\includegraphics[width=0.477\textwidth]{w2wnew.pdf}
\end{figure}

%DO: the attacker does not access sufficient number of lines in eviction set, but accesses eviction set, which is w lines, from an address set
\subsection{Property II: Dynamic Eviction Sets}
\label{security2}
In a contention-based attack, the attacker, after determining an eviction set, accesses it to fill up a cache set, thereby replacing the victim's data. 
%Accessing the eviction set for a specific address is expected to replace the victim's data from the cache due to contention. 
The eviction set is not constant in RollingCache.
%, it does not have lasting eviction sets. 
The addresses that conflict with each other in one \emph{CacheSet} at any given instant may map to different \emph{CacheSets} at another instant, and as soon as just after \emph{W} misses. Thus, there is no replay possible with an eviction set. Discovering an eviction set is made futile by the fact that the attacker's prime and probe result in changing eviction sets. 
%Randomizing caches, on the other hand, try to achieve non-discoverable eviction sets through encryption.

\subsection{Property III: Self and \\Non-Self-Associative Eviction}
\label{security3}
In the final stage of the attack, the attacker relates the misses to one of the accesses in the eviction set.
The evictions in RollingCache on an \emph{AddrSet} are both due to self-associative and non-self-associative addresses. The self-associative evictions result from two consecutive pointer updates, and can evict a maximum of \emph{W} self-associative addresses. With only one \emph{PsPtr}, the past pointer loses track of accesses beyond a single pointer update. However, both the \emph{CacheSets} occupied through the two pointers have possible random evictions from non-self-associative accesses. The duration of the overlapping contention depends on the rate of access to the other \emph{AddrSets}.

The eviction sets still exist and are of different sizes. However, there is no significance to the eviction set under the RollingCache design, i.e., a certain address being evicted does not imply a particular set of addresses might have been accessed by the victim. 
Thus determining the set accessed by the victim upon contention is not possible anymore. 
We prove that the probability of incurring a miss due to a self-associative address is lower than the probability of incurring a miss due to a non-self-associative address.  

Let us consider a RollingCache with `S' \emph{CacheSets}. The number of distinct \emph{AddrSets} is also `S'. Let us say that the attacker tries to determine if the victim accesses a specific \emph{AddrSet} $AddrS_i$. The first phase of the attack constitutes filling both \emph{PrPtr[$AddrS_i$]} and \emph{PsPtr[$AddrS_i$]} \emph{CacheSets} with self-associative addresses from \emph{AddrSet} $AddrS_i$. Finding the set of self-associative addresses also requires the attacker to cause contention on a specific address, from a set of addresses. As seen in the previous subsection, it is not necessary that 2W accesses fill only 2 \emph{CacheSets}. However, the attacker may perform 2W accesses with the expectation to fill up 2 \emph{CacheSets}, allow the victim to execute, and access the same elements from the \emph{AddrSet} $AddrS_i$ accessed before, to see if it incurs a conflict miss. The attacker may or may not incur a miss. In the attacker's prime sequence:
\begin{itemize}
    \item there are possible self evictions, refer Section~\ref{security1}
    \item the victim may cause a miss by accessing a different \emph{AddrSet},
    \item there might be 2 pointer updates, due to which the victim may go undetected even after accessing the same \emph{AddrSet}
    \item and finally the victim may trigger a pointer rollover
\end{itemize}
The only interesting case for the attacker is if the victim access triggers a rollover, as the other cases do not necessarily imply victim's access to the same \emph{AddrSet}. This may be observed as a miss on the least recently used addresses used for prime. It is likely that a first miss in the the least recently used addresses from the prime sequence implies a pointer update, but this cannot be confirmed, as the miss at probe itself can trigger a pointer update, resulting in loss of those accesses. We measure the likelihood that a miss during probe is from victim triggering a pointer rollover in the same \emph{AddrSet}. We determine the probability of the miss being due to the victim's access to \emph{AddrSet} $AddrS_i$.

\emph{\textbf{To find:~}} The probability of the victim's access being from \emph{AddrSet} $AddrS_i$, given a miss is incurred by the attacker, i.e.,  P($AddrS_i|$M).\\
P($AddrS_i$) is the probability of the victim's access being from \emph{AddrSet} $AddrS_i$. %P(M) is the probability of incurring a miss 
%and P($AddrS_i|$M) is the conditional probability of access being from \emph{AddrSet} $AddrS_i$ given that a miss occurred.

The required conditional probability can be determined using Bayes' theorem~\cite{bayes}, which describes the probability of an event in terms of prior knowledge of conditions related to the event. The probability of event $A_i$ occuring given B is true is given as below.
\begin{align}
\label{bayes}
  P(A_i|B)= \frac{P(B|A_i)P(A_i)}{\sum\limits_jP(B|A_j)P(A_j)} 
\end{align}
Using~\ref{bayes}, we get the P($AddrS_i|$M) in terms of the probability of a miss occurring from different \emph{AddrSets} as follows:
\begin{align}
\label{eq2}
  P(AddrS_i|M)= \frac{P(M|AddrS_i)P(AddrS_i)}{\sum\limits_{AddrS_j=1}^SP(M|AddrS_j)P(AddrS_j)} 
\end{align}
Assuming a uniform distribution, the probability of an access being from \emph{AddrSet} $AddrS_i$ is 1/S.  
\begin{align}
\label{eq3}
   P(AddrS_i) = 1/S. 
\end{align}
Similarly,
\begin{align}
\label{eq4}
   P(AddrS_j) = 1/S. 
\end{align}
An access by the victim to  \emph{AddrSet} $AddrS_i$ will result in a miss in the attacker only if the 2 \emph{CacheSets} are completely filled. The likelihood of which is the same as the number of ways (W) in a \emph{CacheSet},i.e.
\begin{align}
\label{eq5}
   P(M|AddrS_i) = (1/W). 
\end{align}


Every \emph{AddrSet} occupies some ways in two different \emph{CacheS-ets}, which implies that there are on average 2 \emph{AddrSets} residing in a \emph{CacheSet}. The probability of incurring a miss in the least recently used accesses from the prime sequence due to an access from some other \emph{AddrSet}, $AddrS_j$, can be given as the probability of \emph{CacheSet} \emph{PsPtr[$AddrS_i$]} being occupied by $AddrS_j$. Since there are $S$ \emph{CacheSets} to choose from, each of these probabilities are $1/S$. 

The attacker's probe access resulting in a miss is likely to coincide with the location of a victim's access 1/W times. Assuming the attacker has the probe resolution of timing a single access by the victim, the 
\begin{align}
\label{eq8}
P(M|AddrS_j) = (1/S)(1/W)
\end{align}
Using~\ref{eq3},~\ref{eq4},~\ref{eq5},~\ref{eq8} in~\ref{eq2} we get,
\begin{align*}
%\label{eq9}
P(AddrS_i|M)= \frac{(\frac{1}{W})(\frac{1}{S})}{(\frac{1}{W})(\frac{1}{S}) + (S-1)(\frac{1}{S})(\frac{1}{W})(\frac{1}{S})}
\end{align*}
\begin{align}
\label{eq10}
=\frac{S}{2S-1}
\end{align}
We can calculate this probability for different number of \emph{CacheSets}. Using `S' = 64 we get,
\begin{align*}
P(AddrS_i|M) = 0.503
\end{align*}

\textcolor{blue}{The above implies that a miss only indicates with a 50\% certainty that the miss was due to the victim accessing the same \emph{AddrSet}, and there is an equal chance that the access was not from the same set. The experiment is as good as a guess based on a flip of a coin. If we consider no attacker control over the victim's accesses, the misses coming from same or a different \emph{AddrSet} are equally likely. This equal likelihood of the access form self and non-self associative addresses along with the difficulties in priming \emph{CacheSets} make iterations of attack to decipher the victim's access ineffective. The above result can be rephrased as, if the attacker manages to start priming the CacheSets at a pointer update, does not self evict his first data entry, and incurs a miss on probe for the first entry, the inference he can make is that the victim's access was either to the same or not to the same \emph{AddrSet} with equal probability. Thus the attack is rendered ineffective in indicating that a miss indeed comes from an access to the same set.}

\textcolor{blue}{The challenges around priming a set comes from being able to start priming at a pointer update, and retaining the first access in the sequence instead of it being replaced by one of the following accesses in the prime sequence. Whether the first access in the prime sequence is not evicted by another access in the prime sequence depends on the availability of invalid cachelines in a given cacheset. The higher the number of valid cachelines in a CacheSet obtained after the pointer update. The less the number of free lines, the higher the probablity of the first access during prime being evicted by one of the accesses in the prime sequence. The quation\ref{eq10} above accounts for the probability of the attacker starting to prime at a pointer update. The effect of the number of invalid cachelines on self eviction at prime makes effective priming further less likely.
}

%There is still a 50\% chance that the attacker incurs a miss due to a victim accessing the same \emph{AddrSet}. Note, however, that we do not consider self-evictions due to random replacement of the attacker's own data during the prime stage for the simplicity of this proof. This implies that the probability of a self-associative eviction by the victim is $<$50\%, which is worse than a coin flip. Another prior work provides a defense by introducing a 50\% error rate in the attack using prefetchers~\cite{prefetcher}.



%We can extend the number of past pointers to more than 2, with increased area and power consumption, and allow lookup in 3 \emph{CacheSets} for an \emph{AddrSet}. The degree of cross contention increases and the performance is expected to increase as well because of continued visibility to the past data. Our evaluation shows a reduction in the probability of self associative eviction to 3.07\% and performance overhead of 0.9\% from using 3 mapping pointers.

%As we see above, self-associative evictions can happen, and so can non-self-associative eviction. Thus the occurrence of a conflict miss does not indicate one or the other.


%If we do not consider an equally likely access from all \emph{AddrSets}, or if the probable \emph{AddrSets} for access are fewer than the total number of \emph{AddrSets}, we can use Equation~\ref{eq10} to calculate the conditional probability with \emph{S} smaller than the total number of \emph{AddrSets}. For \emph{S} = 10, the conditional probability is 0.52, and for \emph{S} = 4, it is 0.57. 
%\textcolor{green}{This 50\% error rate is considering the entire attack sequence comprising of the prime and probe stages, allowing numerous accesses from the attacker.} 

\subsection{Freelist}

The \emph{freelist} is a dynamic structure that allows rotation of \emph{CacheSets} across different \emph{AddrSets}. Its entries are as dynamic as the \emph{AddrSets} that are accessed and undergo pointer update. 
The length of the \emph{freelist} cannot be manipulated by the attacker, as every change to the \emph{freelist} removes an entry and puts an entry on the list, resulting in no net effect on the list length. This means that the attacker cannot reduce the length of the \emph{freelist} to make its behavior deterministic.
Further, the entries on the \emph{freelist} are a microarchitectural state not visible to the attacker: they change at pointer update, i.e. at instants unknown to the attacker. The attacker is not in control of which entries can be put on the \emph{freelist} and at which time, since it depends on the prior metadata (refer \ref{security1}).

An attacker attempting to access a specific \emph{AddrSet} constantly will cause the data from that \emph{AddrSet} to roll over to \emph{CacheSets} that may be picked from the \emph{freelist} on pointer updates. A subsequent access by the victim to any of the other \emph{AddrSets} that were potentially mapped to any of these \emph{CacheSets} prior to the attacker's accesses, may result in a miss. Since these potentially contending \emph{AddrSets} are not known to the attacker, they are unable to disambiguate among the \emph{AddrSets} accessed by the victim. Figure~\ref{freelist} shows a cache with 8 \emph{CacheSets} and a \emph{freelist} of length 2. We discuss a scenario of different pointer updates to demonstrate the effect on an attack. A through H are the \emph{AddrSets}, the mapping pointers are indicated alongside the \emph{AddrSets}, with the \emph{freelist} entries listed at the top of each scenario.
\begin{enumerate}[]
    \item shows random initialization for the mappings and the \emph{freelist}. Accesses occur from different \emph{AddrSets} and their mapping undergoes an update after W cache fills.
    \item shows the instant at which \emph{AddrSet} B undergoes a pointer update, \emph{CacheSet} 5 is picked as the replacement victim, and 3 is added to the \emph{freelist}.
    \item subsequently, the \emph{AddrSet} F undergoes a pointer update, picks \emph{CacheSet} 3, and puts 8 back on the list.
    %\item similarly, G picks \emph{CacheSet} 4 and puts 4 back on the \emph{freelist}.
    \item if the attacker has exclusive access over the cache and is interested in \emph{AddrSet} F, it makes several accesses to \emph{AddrSet} F, effectively moving data between \emph{CacheSets} 3,6,4,8, with any two of these \emph{CacheSets} being accessible at any time.
    \item a subsequent delayed access after a victim's access could be due to contention from \emph{AddrSet} C, E, H, or F (in \emph{CacheSets} 3, 4, 8, 6). We can infer this given the mappings. The attacker however, has no knowledge of the microarchitectural state of the cache, so does not know the smaller set of potentially conflicting \emph{AddrSets} at this instant.
\end{enumerate}
The above illustrates that the attacker's repetitive accesses to the same \emph{AddrSet} does not change the existing mapping of other \emph{AddrSets}. Subsequent conflict misses from the other \emph{AddrSets} mapping to the same \emph{CacheSets} interfere with the attack.

\begin{figure}[tb]
\caption{Accessing a specific \emph{AddrSet} allows \emph{CacheSets} to rotate through the \emph{freelist} but does not change the existing mapping of other \emph{AddrSets} to the same \emph{CacheSets}.}
\label{freelist}
\centering
\includegraphics[width=0.21\textwidth]{freelist.pdf}
\end{figure}

\subsection{AddrSet Cache Footprint}

Figure~\ref{fprint_graph} shows the mapping of different \emph{AddrSets} to \emph{CacheSets} using the \emph{PrPtr}, over 1000 LLC accesses in a sample application (pop2), run with 10 million warmup instructions.  The dots represent the different \emph{AddrSets} on the y-axis that occupy the \emph{CacheSets} on the x-axis. The size of the LLC is 2MB, and it has 2048 \emph{CacheSets}. 
The scatter plot demonstrates how accesses to an \emph{AddrSet} are spread across different \emph{CacheSets}. Figure~\ref{zoom} shows a fewer \emph{AddrSets} and their active \emph{CacheSets}. A closer look into the snapshot shows that a single \emph{CacheSet} 1630 is the active \emph{CacheSet} for 3 different \emph{AddrSets} within the 1000 accesses window.


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=.98\linewidth]{footprint.pdf}
        \caption{Smaller sample showing multiple AddrSet occupancy}
        \label{fprint_graph}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=.98\linewidth]{zoom.pdf}
        \caption{Closer view of the multiple AddrSets mapped to a CacheSet}
        \label{zoom}
    \end{subfigure}
    \caption{Present-Ptr footprint of different \emph{AddrSets}}
    \label{perf}
\end{figure*}


%DO: XXX I think we can move cache flush subsection up, so before footprint
\subsection{Cache Flush}
\textcolor{blue}{
The initial state of the cache is a randomized mapping, with a random number of writes remaining before triggering pointer updates in different \emph{AddrSets}. If the system is being attacked from the very inception, regardless of whether in kernel or user space, the \emph{freelist} is randomly initialized and the indirection pointers would start with a random mapping.
}

\textcolor{blue}{In the case of a cache flush instruction, as the address being flushed may share a \emph{CacheSet} with different \emph{AddrSets} and might not reside in a specific \emph{CacheSet}, the attacker cannot get control of complete \emph{CacheSets} using cache flush instructions. Further, RollingCache retains the state of the indirection pointers (\emph{PrPtr}, \emph{PsPtr}, and all associated metadata) across flushes. When the victim resumes execution, its accesses would continue to be directed to the \emph{CacheSet} pointed to by the \emph{PrPtr} of the accessed \emph{AddrSet} but the number of relocations in the \emph{CacheSet} is not impacted by the flushes. The attacker would not be able to decipher the \emph{AddrSet} that was accessed by the victim  if it incurs a miss in some \emph{CacheSet}.
}


\textcolor{blue}{
\subsection{Robustness against replay attacks}
It has been shown that finding an eviction set for Ceaser-S within the remap interval is possible, because there is a static hashmap within the remap window. Scattercache similarly has a constant set of partially congruent addresses, which once discovered can be reused for launching attacks~\cite{randomattackfix}. Unlike both Scattercache and Ceaser-S, RollingCache does not have specific address sets contending with each other for a specified duration, within which the discovered eviction sets can be reused, rather the mapping updates every W replacements, and we support a maximum of 2W different address lookups. This absence of an epoch is one crucial difference from prior works of defense, blocking discovery or reuse of eviction sets in RollingCache.
The paper attacking Randomized caches uses clflush~\cite{randomattackfix} to reuse the discovered partially congruent eviction sets for priming. Clflush cannot be used to prime a \emph{CacheSet} in Rolling Cache, since we do not write to the same freed lines in a \emph{CacheSet}. The addresses being flushed could be mapped to the \emph{CacheSet} pointed to by the past or the present pointer. The writes after flush continue to contend with yet another address set, since the mapping updates every W replacements. The congruent or partially congruent addresses cannot be reused, as the mapping does not last beyond W accesses. }

\textcolor{blue}{
Further, the attacks on random replacement without filling the cache rely on shared data reuse and the clflush instruction, which is a different threat model compared to contention-based attacks. This work is a defense against contention based attacks, not against reuse based attacks, and is complementary to defense systems built to handle reuse based attacks, such as TimeCache~\cite{timecache}.
}

\textcolor{blue}{
RollingCache uses random replacement. The RELOAD+REFRESH attack~\cite{reloadrefresh} discovers and exploits LRU and other non-random replacement policies. The paper demonstrates attacks that can discover and exploit LRU, Tree PLRU, CLOCK, NRU, Static and Bimodal RRIP, and states that the absence of randomness makes the attacks possible. Given that RollingCache uses random replacement, the RELOAD+REFRESH attack will not be effective. 
Casa is a framework for analyzing random caches and their epochs for their vulnerability and discovery of eviction sets using repeated accesses~\cite{casa}. Since RollingCache has no notion of epoch, does not allow repeated contention on the same address, or in other words does not have a static mapping for a short duration or epoch, the technique in CaSa does not apply to the eviction set inference in RollingCache.
P(AddrSi | M) >> P(AddrSi) for S = 64, but P(AddrSi | M) = P(AddrSi) for S = 2. The equality or inequality of the 2 terms is not indicative of the security of the cache, and the term P(AddrSi | M) is calculated considering P(AddrSi) and other probabilities.
}
